Fully Convolutional Networks and Generative Adversarial Networks Applied to Sclera Segmentation

Due to the world's demand for security systems, biometrics can be seen as an important topic of research in computer vision. One of the biometric forms that has been gaining attention is the recognition based on sclera. The initial and paramount step for performing this type of recognition is the segmentation of the region of interest, i.e. the sclera. In this context, two approaches for such task based on the Fully Convolutional Network (FCN) and on Generative Adversarial Network (GAN) are introduced in this work. FCN is similar to a common convolution neural network, however the fully connected layers (i.e., the classification layers) are removed from the end of the network and the output is generated by combining the output of pooling layers from different convolutional ones. The GAN is based on the game theory, where we have two networks competing with each other to generate the best segmentation. In order to perform fair comparison with baselines and quantitative and objective evaluations of the proposed approaches, we provide to the scientific community new 1,300 manually segmented images from two databases. The experiments are performed on the UBIRIS.v2 and MICHE databases and the best performing configurations of our propositions achieved F-score's measures of 87.48% and 88.32%, respectively.

==> baseline.tex <==
\section{Baseline}
\label{sec:baseline}

==> databases.tex <==
\section{Databases}
\label{sec:databases}

\RL{faltou uma frase de introdução aqui.}

\RL{talvez colocar uma figura com 1 exemplo de cada database pra mostrar pequenas diferenças entre eles? ou não precisa?}

%\noindent
\textbf{\gls*{masdv1}~\cite{das2014sclera}}: the \gls*{masdv1} consists of $2624$ RGB images taken from both eyes of $82$ subjects, i.e., $164$ different eyes. For each eye, four multi-angles (looking straight, left, right and up) are considered. The database consists of $61$ males and $19$ females with different skin and eye ball color, and $4$ of them were wearing contact lenses while providing their eye images. Images were acquired at different times of the day to record the influence on sclera patterns and shapes after prolonged exposure to work and physical stress. The database contains images with blinking, close and blurred eyes. These images were added intentionally to evaluate the segmentation performance in varying non-ideal conditions. High resolution images are provided in the database with $300$ dpi resolution. All the images captured were stored in the JPEG format.


%\textbf{\acrshort*{ubirisv1}\cite{proenca2005ubiris}}: the \acrshort*{ubirisv1} database is composed of $1877$ images collected from $241$ subjects in two distinct sessions. Its most relevant feature is to incorporate images with several noise factors, simulating less constrained image acquisition environments. This enables the evaluation of the robustness of iris recognition methods. For the first image capture session, the enrollment one, the authors tried to minimize noise factors, specially those relative to reflections, luminosity and contrast, capturing images inside a dark room. In the second session, the authors changed the capture place in order to introduce natural luminosity factor. This propitiates the appearance of heterogeneous images with respect to reflections, contrast, luminosity and focus problems. Images collected at this stage simulate the ones captured by a vision system without or with minimal active participation from the subjects, adding several noise problems. These images will be on the recognition stage compared to the ones collected during first session.

\noindent
\textbf{\acrshort*{ubirisv2}}: the \acrshort*{ubirisv2} database used an unconstrained image capturing scheme (at-a-distance and on-the-move) resulting in a highly challenging eye database. Eye images are collected from $261$ subjects for both eyes leading to $522$ classes with two capturing sessions. The capturing distances range from $4$-$8$ meters at a rate of three images per meter with three different iris gaze directions: front, right and left-gaze. The dimension of the captured images is $300\times400$ pixels. We used only images captured at $4$ meters \RL{por quê?}. This database is used in the proposed sclera segmentation evaluation only as this database requires more post-processing on removing noise factors, template alignment and rotation fitting design. \RL{não entendi muito esta última frase.}
	





==> protocol.tex <==
\subsection{Protocol}

To perform the experiments, each of the databases used was divided into the following proportions: $40$\% for training, $20$\% for validation and $40$\% for testing.

Afterward, two test methodologies are applied, one of them uses \gls*{fcn}, and the other uses \gls*{gan}.

\RL{ficou para eu escrever sobre a YOLO. devo fazer isso no ínicio dessa semana.}

==> relatedWork.tex <==
%\section{Related Works}
%\label{sec:related_works}
%
%\subsection{Sclera Based Recognition Systems Where Segmentation Techniques Were Developed}
%
%This section presents the works about sclera based recognition system, where the authors proposed a segmentation methodology to sclera.
%
%
%\cite{Zhou2012} proposed a new concept for human identification, based on sclera vessels pattern. In this work they presents a fully automatic sclera segmentation method for both color and gray-scale images. The sclera region in a color image is estimated using the best representation between two color based techniques, whereas the sclera region in gray-scale image is extracted using Otsu's threshold method. In this work the authors used the UBIRIS V1 dataset and the 
%IUPUI Multiwavelength.
%
%\cite{Das2014} presented in your work a methodology to sclera  sclera segmentation base on time adaptive active contour-based region  growing segmentation method proposed by \cite{902291}. In this methodology the right and left sclera are segmented separately. For region growing-based segmentation, we need a seed point. To find the seed point the authors used the Daugmans integro-diferential method, which is used to calculate the center of iris. From the center of the iris at a distance of 1.1 of the radius length of the iris and a deviation of 45 degrees whit the horizontal, the seed point for region growing is a set in both sides of sclera. In this work the authors used the UBIRIS V1 dataset.
%
%\cite{Kerala2016} presented a a sclera vessels identification based on a single board computer. In this the sclera region is segmented as a rectangular from the hough circular transform applied in iris location. This work don't uses any dataset all the images processed are obtained from a webcam connected to a RaspberryPI.
%
%\subsection{Sclera Segmentation Systems}
%
%In this section are presented the works specifically targeted to sclera segmentation task.
%
%\cite{Das2014} presented a sclera segmentation benchmarking where various research groups proposed their  solutions to solve the problem. In this a total of four teams competed to see what is the best methodology. In This work the authors presented a new dataset name Multi-Angle Sclera Dataset (MASD) version 1. The best presented results are performed by team 4, where the precision and recall values are respectively 95.05\% and 94.56\%.
%
%\cite{Radu2015} presented a novel sclera segmentation algorithm for color images which operates at pixel level. Exploring various color spaces, the proposed approach is robust to image noise and different gaze directions. The algorithm's robustness is enhanced by a two stage classifier. At the first stage, a set of simple classifiers is employed, while at the second stage, a neural network classifier operates on the probabilities space generated by the classifier at the stage 1. The results presents in this as 95.05\% and 94.56\% of precision and recall respectively, theses result are obtained on the MASD v1 dataset.
%
%\cite{Das2016} presented a sclera segmentation and recognition benchmarking where various research groups proposed their  solutions to solve the problem. In this a total of three teams competed to see what is the best methodology. The best presented results are performed by team 1, where the precision and recall values are respectively 85.21\% and 80.21\%.
%
%\cite{Alkassar2016a} proposes a segmentation algorithm which fuses multiple color space skin classifiers to overcome the noise factors introduced through acquiring sclera images such as motion, blur, gaze and rotation. The proposed system is evaluated using UBIRIS V1, UBIRIS V2 an UTIRIS datasets.
%
%\cite{Das2017} presented a sclera segmentation benchmarking where various research groups proposed their  solutions to solve the problem. In this a total of seven teams competed to see what is the best methodology. The best presented results are performed by team 5, where the precision and recall values are respectively 95.34\% and 96.65\%.

\section{Related Work}
\label{sec:related_work}

\RL{falta um parágrafo de introdução do related work. talvez dizendo que é dividido em duas subseções. Quais trabalhos serão descritos (todos? os mais importantes? os que usam abordagens parecidas com a sua?). Acho interessante no final deste parágrafo, citar uns dois surveys (pelo menos 1) interessante para que o leitor possa ir atrás de mais referências.}

\subsection{Sclera-based Recognition Systems Where Segmentation Techniques Were Developed}

This subsection presents works on the sclera-based recognition system, where the authors proposed a new segmentation methodology for sclera.

Zhou et al.~\cite{zhou2012new} proposed a new concept for human identification based on the pattern of sclera vessels. In their work, they presented a fully automated sclera segmentation approach for both color and grayscale images. In color images, the sclera region is estimated using the best representation between two color-based techniques. On the other hand, the Otsu's thresholding method is applied to find the sclera region in grayscale images. The \acrshort*{ubirisv1} and \acrshort*{iupui} databases were used in the experiments. \RL{acho interessante referenciar as bases aqui.}

Das et al.~\cite{das2014sclera} presented a methodology where the right and left sclera are segmented separately. The time adaptive active contour-based region growing segmentation technique proposed by Chan \& Vese~\cite{chan2001active} was employed. The authors applied the Daugman's integro-differential operator to find the seed point required in the region growing-based segmentation. The authors used the \acrshort*{ubirisv1} database in the experiments. \RL{Acho interessante citar Daugman.} 

Delna et al.~\cite{delna2016sclera} presented a sclera identification based on a single-board computer. The sclera region is segmented as a rectangle from the Hough circular transform applied for iris location. This work did not use any public database and all images were obtained from a webcam connected to a Raspberry Pi.

\subsection{Sclera Segmentation Systems}

The works specifically targeted to the sclera segmentation task are presented in this subsection.


Das et al.~\cite{das2014sclera} presented a benchmark for sclera segmentation where four research groups proposed their solutions for this task. All approaches were evaluated in the \gls*{masdv1} database, proposed in the competition. The best results were obtained by Team 4 \RL{citar o trabalho deste grupo? se não tiver, acho que dá pra tirar essa referência à 'Team 4'}, with precision and recall rates of $95.05$\% and $94.56$\%, respectively.

Radu et al.~\cite{radu2015robust} presented a novel sclera segmentation algorithm for color images which operates at pixel-level. Exploring various color spaces, the proposed approach is robust to image noise and different gaze directions. The algorithm's robustness is enhanced by a two-stage classifier. At the first stage, a set of simple classifiers is employed, while at the second stage, a neural network classifier operates on the probabilities space generated by the classifier at the first stage. The reported precision and recall rates were $95.05$\% and $94.56$\%, respectively, on the \gls*{masdv1} database.

\RL{O ideal é juntar os dois parágrafos acima, visto que eles tem ligação.}

Das et al.~\cite{das2016ssrbc} presented a benchmark for sclera segmentation and recognition where three research groups proposed their solutions for this task.\RL{faltou uma frase pra falar o que tem de novo nesse banchmark, por que outro? se for o reconhecimento, dar um enfoque melhor talvez?}. The best results were achieved by Team 1 \RL{citar o trabalho deste grupo? se não tiver, acho que dá pra tirar essa referência à 'Team 1'}, with precision and recall rates of $85.21$\% and $80.21$\%, respectively. \RL{na segmentação ou no reconhecimento?}

Alkassar et al.~\cite{alkassar2016enhanced} proposed a segmentation algorithm which fuses multiple color space skin classifiers to overcome noise introduced by sclera acquisition, such as motion, blur, gaze and rotation. This approach was evaluated using \acrshort*{ubirisv1}, \acrshort*{ubirisv2} an \acrshort*{utiris} databases.

Das et al.~\cite{das2017sserbc} presented a new sclera segmentation benchmark \RL{faltou uma frase pra falar o que tem de novo nesse banchmark, por que outro?} where seven research groups proposed their solutions for this task. The best results were attained by Team 5 \RL{citar o trabalho deste grupo? se não tiver, acho que dá pra tirar essa referência à 'Team 5'}, with precision and recall rates of $95.34$\% and $96.65$\%, respectively.

\subsection{Final Remarks}

\RL{acho que está faltando uma subsection com considerações finais dos trabalhos relacionados. Pontos fracos, pontos em aberto. O que o que você vai fazer tem de diferente (novo) destes trabalhos, etc.}
